Communication-Efficient Variance-Reduced Decentralized Stochastic Optimization over Time-Varying Directed Graphs

We consider the problem of decentralized optimization over time-varying directed networks. The network nodes can access only their local objectives, and aim to collaboratively minimize a global function by exchanging messages with their neighbors. Leveraging sparsification, gradient tracking and variance-reduction, we propose a novel communication-efficient decentralized optimization scheme that is suitable for resource-constrained time-varying directed networks. We prove that in the case of smooth and strongly-convex objective functions, the proposed scheme achieves an accelerated linear convergence rate. To our knowledge, this is the first decentralized optimization framework for time-varying directed networks that achieves such a convergence rate and applies to settings requiring sparsified communication. Experimental results on both synthetic and real datasets verify the theoretical results and demonstrate efficacy of the proposed scheme.

==> tac_analysis.tex <==
For convenience, let us denote the product of a sequence of mixing matrices from time step $s$ to $T$ as 
\begin{equation}
 \bar{M}_m(T:s) = \bar{M}_m^{T} \bar{M}_m^{T-1} \cdots \bar{M}_m^s.
\end{equation}
To further simplify notation, we also introduce
\begin{equation}\label{mproduct1}
M_m((k+1)\mathcal{B}-1:k\mathcal{B}) = \bar{M}_m((k+1)\mathcal{B}-1:k\mathcal{B}) + \gamma F, \end{equation}
and
\begin{equation}
\begin{aligned}
M_m(t:k_1\mathcal{B})
= \bar{M}_m(t:k_2\mathcal{B})M_m(k_2\mathcal{B}-1:(k_2-1)\mathcal{B}) \cdots \\
M_m((k_1+1)\mathcal{B}-1:k_1\mathcal{B}),
\end{aligned}
\end{equation}
where $k_2\mathcal{B} \leq t < (k_2+1)\mathcal{B}-1$ and $k_1, k_2 \in \mathcal{N}, k_1 \leq k_2$. Note that
$M_m((k+1)\mathcal{B}-1:k\mathcal{B})$ is formed by adding a perturbation matrix $\gamma F $ to the product $\bar{M}_m((k+1)\mathcal{B}-1:k\mathcal{B})$.
Finally, we also introduce shorthand notation for the product of weight matrices $B_m$ from time $s$ to $T$,
\begin{equation}
B_m(T:s) = B_m^{T} B_m^{T-1} \cdots B_m^s.
\end{equation}

% {\color{blue}{Modify the algorithm such that the product of column-stochastic matrices $W_{out}$ or $B$ over $\mathcal{B}$ iterations also have non-zero spectral gap.}}

We make several standard assumptions about the graph and network connectivity matrices. These are given next.

\begin{assumption}\label{assumption5}
The product of consecutive mixing matrices $M_m((k+1)\mathcal{B}-1:k\mathcal{B})$ in (\ref{mproduct1}) has a non-zero spectral gap for all $k \geq 0$, $1 \leq m \leq d$, and $0 < \gamma < \gamma_0$ for some $\gamma_0>0$.
\end{assumption}

\begin{remark}
The previous assumption is readily satisfied for a variety of graph structures such as the $\mathcal{B}$-strongly connected directed graph introduced in \cite{nedic2017achieving}, i.e., the union graph over $B$ consecutive graphs starting from time $k\mathcal{B}$ is a strongly connected graph for any non-negative integer $k$.\footnote{There are two versions of the definition of a $\mathcal{B}$-strongly connected directed graph, the difference being the window starting time. Here we consider the definition where the window may start at any time $t = k\mathcal{B}$; this differs from the (more demanding in regards to connectivity) definition in \cite{saadatniaki2018optimization} where the starting time is an arbitrary non-negative integer.}
\end{remark}

%\begin{remark}
%The following network topology examples can satisfy the inequalities in assumptions \ref{assumption5}
%\begin{itemize}
%    \item $\forall t>0, m \in \left\{1, \cdots, d\right\}$, the graph $\G_m(t)=(|n|, \E_m(t))$ is connected, where $\G_m(t)$ models the network connectivity for the $m$-th entry.
%    \item The network is periodically changing and there exists some positive number $B$ such that the union of the directed graphs is strongly-connected for any starting iteration $t$.
%\end{itemize}
%\end{remark}

\begin{assumption}\label{assumption6}
For a fixed $\gamma \in (0, 1)$, the collection of all possible mixing matrices $\{\bar{M}_m^t\}$ is a finite set. {\color{green} Abolfazl: what is $\gamma$? I cannot identify its role in (7)}
%$\{\bar{M}^t$, $\mathcal{U}_M\}$, is a finite set.
\end{assumption}
%Assumption \ref{assumption6} states that after taking into account the effect of randomly sparsified messages on the normalized weight matrices $A_m^t$ and $B_m^t$ and, in turn, the mixing matrix $\bar{M}_m^t$, the set of all possible mixing matrices is finite. 
It is straightforward to verify that Assumption \ref{assumption6} holds for the weight matrices in \eqref{eq:Ws}.

{\color{magenta}{
The following lemma establishes that the difference between the product of mixing matrices and the average matrix has non-zero spectral gap.}}

{\color{blue}{The following lemma establishes the consensus contraction of the product of mixing matrices and the product of normalized weight matrices over $\mathcal{B}$ time steps. }}

{\color{green} Abolfazl: why do we need this lemma in the main text?}
\begin{lemma}\label{lemma1}
Suppose Assumptions \ref{assumption5} and \ref{assumption6} hold. Let $\sigma = \max(|\lambda_{M, 2}|, |\lambda_{B, 2}|)$ denote the larger of the second largest eigenvalues of $M_m((k+1)\mathcal{B}-1:k\mathcal{B} )$ and $B_m((k+1)\mathcal{B}-1:k\mathcal{B})$. Then there exists $\sigma >0$ such that 
\begin{align}
\begin{split}
    \|M_m((k+1)\mathcal{B}-1:k\mathcal{B} ) \z - \Bar{\z} \| \leq \sigma \|\z - \Bar{\z} \|, \ \forall \z \in \R^{2n} \\
    \|B_m((k+1)\mathcal{B}-1:k\mathcal{B} ) \y - \Bar{\y} \| \leq \sigma \|\y - \Bar{\y} \|, \ \forall \y \in \R^{n}, \\
\end{split}
\end{align}
where $\Bar{\z} = [\frac{1}{n}\sum_{i=1}^{2n}z_i, \cdots, \frac{1}{n}\sum_{i=1}^{2n}z_i]^T $ and $\Bar{\y} = [\frac{1}{n}\sum_{i=1}^{n}y_i, \cdots, \frac{1}{n}\sum_{i=1}^{n}y_i]^T $. 
{\color{green} Abolfazl: maybe state here that $\sigma$ depends on $q = k/d$. Or even change it to $\sigma_q$?}
\end{lemma}

\begin{proof}
The result follows directly from Lemma $2$ in \cite{chen2020communication} and the column-stochasticity of $M_m((k+1)\mathcal{B}-1:k\mathcal{B} )$.
\end{proof}


%----------------------------------------

%\begin{assumption}\label{assumption2}
%The objective function $f$ is $\mu$-strongly-convex, i.e. $\forall \x_1, \x_2 \in \R^d$ and for some $\mu >0$, 
%\begin{equation*}
%    f(\x_2) \geq f(\x_1) + \langle \nabla f(\x_1), \x_2 - \x_1 \rangle + \frac{\mu}{2} \|\x_2 - \x_1 \|^2
%\end{equation*}
%\end{assumption}

%\begin{assumption}\label{assumption3}
%Each component of local objective function $f_{i, j}$ is $L$-smooth, i.e.
%$\forall \x_1, \x_2 \in \R^d$ and for some $L >0$,
%\begin{equation*}
%    \|\nabla f_{i, j}(\x_1) - \nabla f_{i, j}(\x_2) \| \leq L\|\x_1 - \x_2 \|
%\end{equation*}
%\end{assumption}

%If the assumptions \ref{assumption2} and \ref{assumption3} hold, then we can derive that $f$ is also $L$-smooth and $L \geq \mu$. Let us denote $\Tilde{Q} = \frac{L}{\mu}$ as the condition number of $f$. 

\begin{assumption}\label{assumption4}
There exists $D>0$ such that 
$\forall i \in \left\{1, \cdots, n \right\}$, $m \in \left\{1, \cdots, d \right\}$ and $t>0$, it holds that $|g_{im}^t|<D$.
\end{assumption}
{\color{green} Abolfazl: we should be more than ready for concerns regarding this assumption.}

 %-----------------------------


\begin{theorem}
Suppose Assumptions~1-3 hold. Let each component of the local objective function $f_{i, j}$ be $L$-smooth\footnote{This implies that
$\forall \x_1, \x_2 \in \R^d$ there exists $L >0$ such that
%\begin{equation*}
    $\|\nabla f_{i, j}(\x_1) - \nabla f_{i, j}(\x_2) \| \leq L\|\x_1 - \x_2 \|$.
%\end{equation*}
}
and the objective $f$ be $\mu$-strongly-convex\footnote{In other words, $\forall \x_1, \x_2 \in \R^d$ there exists $\mu >0$ such that
%\begin{equation*}
    $f(\x_2) \geq f(\x_1) + \langle \nabla f(\x_1), \x_2 - \x_1 \rangle + \frac{\mu}{2} \|\x_2 - \x_1 \|^2$.
%\end{equation*}
}; 
denote the condition number of $f$ by $\Tilde{Q} = \frac{L}{\mu}$. If the step size $\alpha$ and the inner-loop length $T$ satisfy
\begin{equation*}
%    \alpha = O((\frac{1-\sigma^2)^2}{\Tilde{Q}}), \quad 
%    T = O(\frac{\Tilde{Q}^2 \log \Tilde{Q}}{(1-\sigma^2)^2})
\alpha = \frac{(1-\sigma^2)^2}{187\tilde{Q} L}, \;\;\;
 T = \mathcal{B} \lceil \frac{748\Tilde{Q}^2}{(1-\sigma^2)^2 \mathcal{B}}\log (200\Tilde{Q}^2) \rceil,
\end{equation*}
the proposed algorithm achieves linear convergence.
Specifically,
to reach $\epsilon$-accuracy, Algorithm \ref{alg:B} takes at most $\O(\frac{\Tilde{Q}^2\ln \Tilde{Q}}{(1-\sigma^2)^2}\ln 1/\epsilon)$ communication rounds and performs $\O(\frac{\Tilde{Q}^2\ln \Tilde{Q}}{(1-\sigma^2)^2\mathcal{B}}\ln 1/\epsilon)$ gradient computation.
{\color{green} Abolfazl: The dependence on $D$ is not clear. Also, can $S$ take any value?}
\end{theorem}

To prove the convergence rate stated in the theorem, we need to analyze dynamics and establish convergence of the optimality gap, i.e., the difference between the current state and the optimal state (a technique akin to the approach in \cite{nedic2017achieving, xin2019variance}). A critical step in this analysis is to show that the product of mixing matrices guides the local vectors towards the average consensus, as stated in Lemma~1. Following this result, we proceed to find convergence rate of the stochastic variance-reduced method used by the proposed algorithm and thus finalize the proof of Theorem~1. Details of the proof are provided in Appendix.

\begin{remark}
Clearly, the communication cost of Algorithm \ref{alg:B} depends on the level of sparsification, i.e., the value of parameter $k$. Intuitively, if agents communicate fewer entries in each round, the communication cost per round decreases but the algorithm may take more rounds to reach the same accuracy. Therefore, the total communication cost until reaching a pre-specified $\epsilon$-accuracy, found as the product of the number of communication rounds and the cost per round, is of interest. Let $q$ denote the fraction of entries being communicated per iteration; smaller $q$ implies more aggressive sparsification. This compression level parameter, $q$, impacts $\sigma$ in Theorem~1; in particular, for a fixed network connectivity parameter $\mathcal{B}$, smaller $q$ leads to sparser mixing matrices and, consequently, greater $\sigma$. Note that large $\mathcal{B}$ may be caused by sparsity of the instances of a time-varying network, thus leading to large values of $\sigma$. {\color{green} Abolfazl: maybe cite our semi-analysis for random graphs in [14]?}
\end{remark} 




==> tac_bib.tex <==
\begin{thebibliography}{00}
@manual{kaggle,
  title  = "The Stack Overflow Data",
  url    = "https://www.kaggle.com/stackoverflow/stackoverflow",
}
@article{
koloskova2019decentralizeda,
  title={Decentralized deep learning with arbitrary communication compression},
  author={Koloskova, Anastasia and Lin, Tao and Stich, Sebastian U and Jaggi, Martin},
  journal={arXiv preprint arXiv:1907.09356},
  year={2019}
}

@inproceedings{stich2018sparsified,
  title={Sparsified {SGD} with memory},
  author={Stich, Sebastian U and Cordonnier, Jean-Baptiste and Jaggi, Martin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4447--4458},
  year={2018}
}
@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}
@inproceedings{tang2018communication,
  title={Communication compression for decentralized training},
  author={Tang, Hanlin and Gan, Shaoduo and Zhang, Ce and Zhang, Tong and Liu, Ji},
  booktitle={Advances in Neural Information Processing Systems},
  pages={7652--7662},
  year={2018}
}
@article{benaych2019largest,
  title={Largest eigenvalues of sparse inhomogeneous Erd{\H{o}}s--R{\'e}nyi graphs},
  author={Benaych-Georges, Florent and Bordenave, Charles and Knowles, Antti and others},
  journal={The Annals of Probability},
  volume={47},
  number={3},
  pages={1653--1676},
  year={2019},
  publisher={Institute of Mathematical Statistics}
}
@inproceedings{koloskova2019decentralized,
  title={Decentralized Stochastic Optimization and Gossip Algorithms with Compressed Communication},
  author={Koloskova, Anastasia and Stich, Sebastian and Jaggi, Martin},
  booktitle={International Conference on Machine Learning},
  pages={3478--3487},
  year={2019}
}
@article{erdos1959random,
  title={On random graphs},
  author={Erd{\"o}s, Paul and R{\'e}nyi, Alfr{\'e}d and others},
  journal={Publicationes mathematicae},
  volume={6},
  number={26},
  pages={290--297},
  year={1959}
}
@inproceedings{shen2018towards,
  title={Towards More Efficient Stochastic Decentralized Learning: {F}aster Convergence and Sparse Communication},
  author={Shen, Zebang and Mokhtari, Aryan and Zhou, Tengfei and Zhao, Peilin and Qian, Hui},
  booktitle={International Conference on Machine Learning},
  pages={4624--4633},
  year={2018}
}
@article{nedic2017achieving,
  title={Achieving geometric convergence for distributed optimization over time-varying graphs},
  author={Nedic, Angelia and Olshevsky, Alex and Shi, Wei},
  journal={SIAM Journal on Optimization},
  volume={27},
  number={4},
  pages={2597--2633},
  year={2017},
  publisher={SIAM}
}
@inproceedings{kempe2003gossip,
  title={Gossip-based computation of aggregate information},
  author={Kempe, David and Dobra, Alin and Gehrke, Johannes},
  booktitle={44th Annual IEEE Symposium on Foundations of Computer Science, 2003. Proceedings.},
  pages={482--491},
  year={2003},
  organization={IEEE}
}
@inproceedings{reisizadeh2019robust,
  title={Robust and communication-efficient collaborative learning},
  author={Reisizadeh, Amirhossein and Taheri, Hossein and Mokhtari, Aryan and Hassani, Hamed and Pedarsani, Ramtin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={8386--8397},
  year={2019}
}

@article{nedic2014distributed,
  title={Distributed optimization over time-varying directed graphs},
  author={Nedi{\'c}, Angelia and Olshevsky, Alex},
  journal={IEEE Transactions on Automatic Control},
  volume={60},
  number={3},
  pages={601--615},
  year={2014},
  publisher={IEEE}
}
@article{jadbabaie2003coordination,
  title={Coordination of groups of mobile autonomous agents using nearest neighbor rules},
  author={Jadbabaie, Ali and Lin, Jie and Morse, A Stephen},
  journal={IEEE Transactions on automatic control},
  volume={48},
  number={6},
  pages={988--1001},
  year={2003},
  publisher={IEEE}
}
@article{ren2005consensus,
  title={Consensus seeking in multiagent systems under dynamically changing interaction topologies},
  author={Ren, Wei and Beard, Randal W},
  journal={IEEE Transactions on automatic control},
  volume={50},
  number={5},
  pages={655--661},
  year={2005},
  publisher={IEEE}
}
@article{ren2007information,
  title={Information consensus in multivehicle cooperative control},
  author={Ren, Wei and Beard, Randal W and Atkins, Ella M},
  journal={IEEE Control systems magazine},
  volume={27},
  number={2},
  pages={71--82},
  year={2007},
  publisher={IEEE}
}
@inproceedings{mcmahan2017communication,
  title={Communication-Efficient Learning of Deep Networks from Decentralized Data},
  author={McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and y Arcas, Blaise Aguera},
  booktitle={Artificial Intelligence and Statistics},
  pages={1273--1282},
  year={2017}
}

@techreport{tsitsiklis1984problems,
  title={Problems in decentralized decision making and computation.},
  author={Tsitsiklis, John Nikolas},
  year={1984},
  institution={Massachusetts Inst of Tech Cambridge Lab for Information and Decision Systems}
}

@article{boyd2006randomized,
  title={Randomized gossip algorithms},
  author={Boyd, Stephen and Ghosh, Arpita and Prabhakar, Balaji and Shah, Devavrat},
  journal={IEEE transactions on information theory},
  volume={52},
  number={6},
  pages={2508--2530},
  year={2006},
  publisher={IEEE}
}

@article{xiao2004fast,
  title={Fast linear iterations for distributed averaging},
  author={Xiao, Lin and Boyd, Stephen},
  journal={Systems \& Control Letters},
  volume={53},
  number={1},
  pages={65--78},
  year={2004},
  publisher={Elsevier}
}

@article{nedic2009distributed,
  title={Distributed subgradient methods for multi-agent optimization},
  author={Nedic, Angelia and Ozdaglar, Asuman},
  journal={IEEE Transactions on Automatic Control},
  volume={54},
  number={1},
  pages={48--61},
  year={2009},
  publisher={IEEE}
}

@article{johansson2010randomized,
  title={A randomized incremental subgradient method for distributed optimization in networked systems},
  author={Johansson, Bj{\"o}rn and Rabi, Maben and Johansson, Mikael},
  journal={SIAM Journal on Optimization},
  volume={20},
  number={3},
  pages={1157--1170},
  year={2010},
  publisher={SIAM}
}

@inproceedings{wei2012distributed,
  title={Distributed alternating direction method of multipliers},
  author={Wei, Ermin and Ozdaglar, Asuman},
  booktitle={2012 IEEE 51st IEEE Conference on Decision and Control (CDC)},
  pages={5445--5450},
  year={2012},
  organization={IEEE}
}

@article{duchi2011dual,
  title={Dual averaging for distributed optimization: {C}onvergence analysis and network scaling},
  author={Duchi, John C and Agarwal, Alekh and Wainwright, Martin J},
  journal={IEEE Transactions on Automatic control},
  volume={57},
  number={3},
  pages={592--606},
  year={2011},
  publisher={IEEE}
}

@inproceedings{nedic2015decentralized,
  title={Decentralized online optimization with global objectives and local communication},
  author={Nedi{\'c}, Angelia and Lee, Soomin and Raginsky, Maxim},
  booktitle={2015 American Control Conference (ACC)},
  pages={4497--4503},
  year={2015},
  organization={IEEE}
}

@inproceedings{he2018cola,
  title={Cola: {D}ecentralized linear learning},
  author={He, Lie and Bian, An and Jaggi, Martin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4536--4546},
  year={2018}
}

@article{xi2017distributed,
  title={On the distributed optimization over directed networks},
  author={Xi, Chenguang and Wu, Qiong and Khan, Usman A},
  journal={Neurocomputing},
  volume={267},
  pages={508--515},
  year={2017},
  publisher={Elsevier}
}
@inproceedings{cai2011average,
  title={Average consensus on general digraphs},
  author={Cai, Kai and Ishii, Hideaki},
  booktitle={2011 50th IEEE Conference on Decision and Control and European Control Conference},
  pages={1956--1961},
  year={2011},
  organization={IEEE}
}

@article{cai2014average,
  title={Average consensus on arbitrary strongly connected digraphs with time-varying topologies},
  author={Cai, Kai and Ishii, Hideaki},
  journal={IEEE Transactions on Automatic Control},
  volume={59},
  number={4},
  pages={1066--1071},
  year={2014},
  publisher={IEEE}
}

@inproceedings{zhang2017zipml,
  title={Zipml: {T}raining linear models with end-to-end low precision, and a little bit of deep learning},
  author={Zhang, Hantian and Li, Jerry and Kara, Kaan and Alistarh, Dan and Liu, Ji and Zhang, Ce},
  booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  pages={4035--4043},
  year={2017},
  organization={JMLR. org}
}

@inproceedings{wen2017terngrad,
  title={Terngrad: {T}ernary gradients to reduce communication in distributed deep learning},
  author={Wen, Wei and Xu, Cong and Yan, Feng and Wu, Chunpeng and Wang, Yandan and Chen, Yiran and Li, Hai},
  booktitle={Advances in neural information processing systems},
  pages={1509--1519},
  year={2017}
}

@article{cai2012average,
  title={Average consensus on general strongly connected digraphs},
  author={Cai, Kai and Ishii, Hideaki},
  journal={Automatica},
  volume={48},
  number={11},
  pages={2750--2761},
  year={2012},
  publisher={Elsevier}
}

@article{nedic2016stochastic,
  title={Stochastic gradient-push for strongly convex functions on time-varying directed graphs},
  author={Nedi{\'c}, Angelia and Olshevsky, Alex},
  journal={IEEE Transactions on Automatic Control},
  volume={61},
  number={12},
  pages={3936--3947},
  year={2016},
  publisher={IEEE}
}

@article{saadatniaki2018optimization,
  title={Optimization over time-varying directed graphs with row and column-stochastic matrices},
  author={Saadatniaki, Fakhteh and Xin, Ran and Khan, Usman A},
  journal={arXiv preprint arXiv:1810.07393},
  year={2018}
}

@article{xin2019distributed,
  title={Distributed stochastic optimization with gradient tracking over strongly-connected networks},
  author={Xin, Ran and Sahu, Anit Kumar and Khan, Usman A and Kar, Soummya},
  journal={arXiv preprint arXiv:1903.07266},
  year={2019}
}

@article{schmidt2017minimizing,
  title={Minimizing finite sums with the stochastic average gradient},
  author={Schmidt, Mark and Le Roux, Nicolas and Bach, Francis},
  journal={Mathematical Programming},
  volume={162},
  number={1-2},
  pages={83--112},
  year={2017},
  publisher={Springer}
}

@inproceedings{johnson2013accelerating,
  title={Accelerating stochastic gradient descent using predictive variance reduction},
  author={Johnson, Rie and Zhang, Tong},
  booktitle={Advances in neural information processing systems},
  pages={315--323},
  year={2013}
}

@article{chen2020communication1,
  title={Communication-Efficient Algorithms for Decentralized Optimization Over Time-Varying Directed Graphs},
  author={Chen, Yiuye and Hashemi, Abolfazl and Vikalo, Haris},
  journal={arXiv preprint arXiv:2005.13189},
  year={2020}
}
@article{hashemi2020delicoco,
	title={On the Benefits of Multiple Gossip Steps in Communication-Constrained Decentralized Optimization},
	author={Hashemi, Abolfazl and Acharya, Anish and Das, Rudrajit and Vikalo, Haris and Sanghavi, Sujay and Dhillon, Inderjit},
	journal={arXiv preprint arXiv:2012.04061},
	year={2020}
}

@inproceedings{taheriquantized,
  title={Quantized Decentralized Stochastic Learning over Directed Graphs},
  author={Taheri, Hossein and Mokhtari, Aryan and Hassani, Hamed and Pedarsani, Ramtin},
  booktitle={International Conference on Machine Learning (ICML)},
  year={2020}
}

@article{ram2010distributed,
  title={Distributed stochastic subgradient projection algorithms for convex optimization},
  author={Ram, S Sundhar and Nedi{\'c}, Angelia and Veeravalli, Venugopal V},
  journal={Journal of optimization theory and applications},
  volume={147},
  number={3},
  pages={516--545},
  year={2010},
  publisher={Springer}
}
@article{das2020improved,
  title={Improved Convergence Rates for Non-Convex Federated Learning with Compression},
  author={Das, Rudrajit and Hashemi, Abolfazl and Sanghavi, Sujay and Dhillon, Inderjit S},
  journal={arXiv preprint arXiv:2012.04061},
  year={2020}
}

@article{xin2019variance,
  title={Variance-reduced decentralized stochastic optimization with accelerated convergence},
  author={Xin, Ran and Khan, Usman A and Kar, Soummya},
  journal={arXiv preprint arXiv:1912.04230},
  year={2019}
}

@inproceedings{li2020communication,
  title={Communication-efficient distributed optimization in networks with gradient tracking and variance reduction},
  author={Li, Boyue and Cen, Shicong and Chen, Yuxin and Chi, Yuejie},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={1662--1672},
  year={2020},
  organization={PMLR}
}

@article{qu2017harnessing,
  title={Harnessing smoothness to accelerate distributed optimization},
  author={Qu, Guannan and Li, Na},
  journal={IEEE Transactions on Control of Network Systems},
  volume={5},
  number={3},
  pages={1245--1260},
  year={2017},
  publisher={IEEE}
}

@inproceedings{gharesifard2010does,
  title={When does a digraph admit a doubly stochastic adjacency matrix?},
  author={Gharesifard, Bahman and Cort{\'e}s, Jorge},
  booktitle={Proceedings of the 2010 American Control Conference},
  pages={2440--2445},
  year={2010},
  organization={IEEE}
}

@inproceedings{chen2020communication,
  title={Decentralized Optimization on Time-Varying Directed Graphs Under Communication Constraints},
  author={Chen, Yiyue and Hashemi, Abolfazl and Vikalo, Haris},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3670--3674},
  year={2021},
  organization={IEEE}
}

@article{chen2021communication,
  title={Communication-Efficient Variance-Reduced Decentralized Stochastic Optimization over Time-Varying Directed Graphs},
  author={Chen, Yiyue and Hashemi, Abolfazl and Vikalo, Haris},
  journal={arXiv preprint arXiv:2101.09583},
  year={2021}
}

@article{qureshi2021push,
  title={Push-SAGA: A decentralized stochastic algorithm with variance reduction over directed graphs},
  author={Qureshi, Muhammad I and Xin, Ran and Kar, Soummya and Khan, Usman A},
  journal={IEEE Control Systems Letters},
  year={2021},
  publisher={IEEE}
}


\end{thebibliography}

%-------------------


